Segmental Advantage Estimation: Enhancing PPO for Long-Context LLM Training

Training Large Language Models (LLMs) for reasoning tasks is increasingly driven by Reinforcement Learning with Verifiable Rewards (RLVR), where Proximal Policy Optimization (PPO) provides a principled framework for stable policy updates. However, the practical application of PPO is hindered by unreliable advantage estimation in the sparse-reward RLVR regime. This issue arises because the sparse rewards in RLVR lead to inaccurate intermediate value predictions, which in turn introduce significant bias when aggregated at every token by Generalized Advantage Estimation (GAE). To address this, we introduce Segmental Advantage Estimation (SAE), which mitigates the bias that GAE can incur in RLVR. Our key insight is that aggregating $n$-step advantages at every token(as in GAE) is unnecessary and often introduces excessive bias, since individual tokens carry minimal information. Instead, SAE first partitions the generated sequence into coherent sub-segments using low-probability tokens as heuristic boundaries. It then selectively computes variance-reduced advantage estimates only from these information-rich segment transitions, effectively filtering out noise from intermediate tokens. Our experiments demonstrate that SAE achieves superior performance, with marked improvements in final scores, training stability, and sample efficiency. These gains are shown to be consistent across multiple model sizes, and a correlation analysis confirms that our proposed advantage estimator achieves a higher correlation with an approximate ground-truth advantage, justifying its superior performance.

==> related_work_bkp.tex <==
\paragraph{Reinforcement learning for large language models} has emerged as a critical paradigm for aligning language models with human preferences, primarily through Reinforcement Learning from Human Feedback (RLHF). The foundational work by  \citep{schulman2017proximal} introduced Proximal Policy Optimization (PPO), which became the backbone of modern language model alignment due to its stability compared to other policy gradient methods. This approach was first successfully scaled to large language models by \citep{christiano2017deep}, who demonstrated preference-based reward learning, and later by \citep{ouyang2022training} in their seminal InstructGPT work.
In the RLVR domain, recent advances like DeepSeek-R1 \citep{deepseek2025r1} have shown the potential of LLM in reasoning tasks. They typically trains LLM using  Group Relative Policy Optimization (GRPO), which forgoes token-level credit assignment by operating on sequence-level rewards. 
While this approach simplifies implementation, recent studies have shown that PPO can achieve superior performance \citep{vapo,hu2025openreasonerzero}. This suggests that the granular credit assignment mechanism of PPO provides some advantage, making it a direction with potentially greater upside for RLVR tasks.

\paragraph{Advantage estimation methods} form the core of policy gradient algorithms PPO, with Generalized Advantage Estimation (GAE) \citep{schulman2015high} providing the dominant framework for reducing variance in policy gradient estimates through exponentially-weighted temporal difference estimates. 
% GAE addresses the fundamental bias-variance tradeoff in advantage estimation by introducing a $\lambda$ parameter that interpolates between high-bias, low-variance temporal difference estimates and low-bias, high-variance Monte Carlo returns. 
% However, standard GAE faces significant limitations when applied to long sequences, as highlighted in recent theoretical analysis of credit assignment problems \citep{pignatelli2024survey}. 
% Several recent works have proposed improvements to address these limitations: \citep{jin2023partial} introduce partial advantage estimation to reduce truncation bias in finite-length trajectories, while \citep{shaik2025generalized} extend GAE to distributional reinforcement learning using Wasserstein metrics. 
Alternative approaches like Direct Advantage Estimation \citep{pan2022direct} eliminate the need for separate value functions by modeling advantages directly from causal effects, though these methods still operate at the token level. 
The emergence of language-based value functions \citep{liu2024natural} represents a paradigm shift toward more interpretable advantage estimation, but current methods lack the hierarchical structure needed for effective long-context processing.

==> texts/proof_thm_bias.tex <==

\textbf{Step 1: Exact bias decomposition via telescoping}

From the SAE formulation, the bias contribution is:
\begin{equation}
\text{bias}_{A_0^{\text{SAE}}} = \sum_{l=0}^{T-1} \left(\prod_{i=0}^{l-1} \lambda_{\text{SAE}}(i)\right) [\varepsilon(s_{l+1}) - \varepsilon(s_l)]
\end{equation}

For uniform segmentation, we partition the sum by segments $S_k = [kM, (k+1)M)$ for $k = 0, 1, \ldots, T/M-1$:
\begin{align}
\text{bias}_{A_0^{\text{SAE}}} &= \sum_{k=0}^{T/M-1} \sum_{l=kM}^{(k+1)M-1} \lambda^k [\varepsilon(s_{l+1}) - \varepsilon(s_l)] \\
&= \sum_{k=0}^{T/M-1} \lambda^k [\varepsilon(s_{(k+1)M}) - \varepsilon(s_{kM})]
\end{align}

where we used the telescoping property within each segment and $\prod_{i=0}^{kM-1} \lambda_{\text{SAE}}(i) = \lambda^k$.

\textbf{Step 2: Rearrangement and cancellation structure}

Expanding the telescoping sum:
\begin{align}
\text{bias}_{A_0^{\text{SAE}}} &= [\varepsilon(s_M) - \varepsilon(s_0)] + \lambda[\varepsilon(s_{2M}) - \varepsilon(s_M)] \\
&\quad + \lambda^2[\varepsilon(s_{3M}) - \varepsilon(s_{2M})] + \ldots + \lambda^{T/M-1}[\varepsilon(s_T) - \varepsilon(s_{(T/M-1)M})]
\end{align}

Collecting terms by $\varepsilon(s_{kM})$ coefficients:
\begin{align}
\text{bias}_{A_0^{\text{SAE}}} &= -\varepsilon(s_0) + \varepsilon(s_M)(1-\lambda) + \varepsilon(s_{2M})\lambda(1-\lambda) \\
&\quad + \varepsilon(s_{3M})\lambda^2(1-\lambda) + \ldots + \varepsilon(s_{(T/M-1)M})\lambda^{T/M-2}(1-\lambda) + \lambda^{T/M-1}\varepsilon(s_T)
\end{align}

Under the assumption $\varepsilon(s_T) = 0$, we obtain:
\begin{equation}
\text{bias}_{A_0^{\text{SAE}}} = -\varepsilon(s_0) + \sum_{k=1}^{T/M-1} \lambda^{k-1} (1-\lambda) \varepsilon(s_{kM})
\end{equation}

\textbf{Step 3: Upper bound derivation}

Applying the triangle inequality and error bound assumption:
\begin{align}
\left|\text{bias}_{A_0^{\text{SAE}}}\right| &\leq |\varepsilon(s_0)| + \sum_{k=1}^{T/M-1} \lambda^{k-1} (1-\lambda) |\varepsilon(s_{kM})| \\
&\leq \alpha \exp\left(\frac{T}{\beta}\right) + (1-\lambda) \sum_{k=1}^{T/M-1} \lambda^{k-1} \alpha \exp\left(\frac{T-kM}{\beta}\right) \\
&= \alpha \exp\left(\frac{T}{\beta}\right) \left[1 + (1-\lambda) \sum_{k=1}^{T/M-1} \lambda^{k-1} \exp\left(\frac{-kM}{\beta}\right)\right]
\end{align}

For the geometric series with $\mu = \lambda \exp\left(\frac{-M}{\beta}\right) < 1$:
\begin{equation}
\sum_{k=1}^{T/M-1} \lambda^{k-1} \exp\left(\frac{-kM}{\beta}\right) = \lambda^{-1}\sum_{k=1}^{T/M-1} \mu^k \leq \sum_{k=1}^{\infty} \mu^k = \frac{\mu}{\lambda(1-\mu)} = \frac{\exp\left(\frac{-M}{\beta}\right)}{1 - \lambda\exp\left(\frac{-M}{\beta}\right)}
\end{equation}

Therefore:
\begin{equation}
\left|\text{bias}_{A_0^{\text{SAE}}}\right| \leq \alpha \exp\left(\frac{T}{\beta}\right) \left[1 + \frac{(1-\lambda)\exp\left(\frac{-M}{\beta}\right)}{1 - \lambda \exp\left(\frac{-M}{\beta}\right)}\right]
= \alpha \exp\left(\frac{T}{\beta}\right) \left[1 + \frac{1-\lambda}{\exp\left(\frac{M}{\beta}\right) - \lambda}\right]
\end{equation}
